Permissive Controller Synthesis for Probabilistic Systems

We propose novel controller synthesis techniques for probabilistic systems modelled using stochastic two-player games: one player acts as a controller, the second represents its environment, and probability is used to capture uncertainty arising due to, for example, unreliable sensors or faulty system components. Our aim is to generate robust controllers that are resilient to unexpected system changes at runtime, and flexible enough to be adapted if additional constraints need to be imposed. We develop a permissive controller synthesis framework, which generates multi-strategies for the controller, offering a choice of control actions to take at each time step. We formalise the notion of permissivity using penalties, which are incurred each time a possible control action is disallowed by a multi-strategy. Permissive controller synthesis aims to generate a multi-strategy that minimises these penalties, whilst guaranteeing the satisfaction of a specified system property. We establish several key results about the optimality of multi-strategies and the complexity of synthesising them. Then, we develop methods to perform permissive controller synthesis using mixed integer linear programming and illustrate their effectiveness on a selection of case studies.

==> prelims.tex <==
%\vspace*{-0.2cm}
\section{Preliminaries}\label{sec:prelims}
%\vspace*{-0.1cm}

We denote by $\Dist(X)$ the set of discrete probability distributions over a set $X$.
A \emph{Dirac} distribution is one that assigns probability 1 to some $s\in X$.
%
The \emph{support} of a distribution $d\in\Dist(X)$ 
is defined as $\support{d} \rmdef \{x\in X \mid d(x) > 0\}$.
%to denote the set of element for which $d$ is non-zero.

%Given a set $X$, we use $\Dist(X)$ to denote the set of all discrete probability
%distributions over $X$. For $d\in \Dist(X)$, we use $\support{d} \rmdef \{x\in X \mid d(x) > 0\}$
%to denote the set of element for which $d$ is non-zero. A distribution
%$d$ with support $\{x_1,\dots,x_n\}$ and $d(x_i)=\lambda_i$ will also
%be written as $\lambda_1x_1+\dots+\lambda_nx_n$; in particular, a
%Dirac distribution, i.e. $d\in\Dist(X)$ such that for some $x$ we
%have $d(x)=1$, will simply be written as $x$.

%-------------------------------------------------------------------------

\subsection{Stochastic Games}
%
In this paper, we use \emph{turn-based stochastic two-player games},
which we often refer to simply as \emph{stochastic games}. % or just \emph{games}.
%
%\begin{defi}[Stochastic game]\label{defn:stochgame}
A stochastic game takes the form $\sgame=\gametuple$,
where $S\rmdef S_\Diamond\cup S_\Box$ is a finite set of states, each associated with
player $\Diamond$ or $\Box$, $\sinit\in S$ is an initial state, $\act$ is a finite set of actions and
$\delta : S {\times} \act \rightarrow \Dist(S)$ is a (partial) probabilistic transition function such that
the distributions assigned by $\delta$ only select elements of $S$ with rational probabilities.
%\end{defi}

An MDP is a stochastic game %$\sgame=\gametuple$ % with $S_\Box = \emptyset$.
in which either $S_\Diamond$ or $S_\Box$ is empty.
%
Each state $s$ of a stochastic game $\sgame$ has a set %$\enab{s}$
of \emph{enabled} actions,
given by $\enab{s}\rmdef\{a\in\act \,|\, \delta(s,a)\mbox{ is defined}\}$.
The %player who owns state $s$ (the unique player $\eitherplayer$ such that $s\in S_\eitherplayer$)
unique player $\eitherplayer\in\{\Diamond,\Box\}$ such that $s\in S_{\eitherplayer}$
picks an action $a\in\enab{s}$ to be taken in state $s$.
Then, the next state is determined randomly according
to the distribution $\delta(s,a)$, i.e., a transition to state $s'$ occurs with probability $\delta(s,a)(s')$.

A \emph{path} through $\sgame$ is a (finite or infinite) sequence $\omega=s_0 a_0 s_1 a_1 \dots$,
where $s_i\in S$, $a_i\in\enab{s_i}$ and $\delta(s_i,a_i)(s_{i+1})>0$ for all $i$.
We denote by $\ipaths_s$ the set of all infinite paths starting in state $s$.
For a player $\eitherplayer\in\{\Diamond,\Box\}$, we denote by
$\fpaths^\eitherplayer$ the set of all finite paths starting in any state and ending in a state from $S_\eitherplayer$.
%and, for finite $\omega$, $\last(\omega)$ is its last state. % was only used once

A \emph{strategy}
$\sigma:\fpaths^\eitherplayer \rightarrow \dist(\act)$
for player $\eitherplayer$
of $\sgame$ is a resolution of the choices of actions in each state
from $S_\eitherplayer$ based on the execution so far,
such that only enabled actions in a state are chosen with non-zero probability.
In standard fashion \cite{KSK76}, a pair of strategies $\sigma$ and
$\pi$ for $\Diamond$ and $\Box$ induces, for any state $s$, a probability measure
$\Prb_{\sgame,s}^{\sigma,\pi}$ over $\ipaths_s$.
%As above, we simply write  $\Prb_{\sgame}^{\sigma,\pi}$ for $\Prb_{\sgame,\sinit}^{\sigma,\pi}$.
%
A strategy $\sigma$ is \emph{deterministic} if $\sigma(\omega)$ is a Dirac distribution
for all $\omega$, and \emph{randomised} if not.
In this work, we focus purely on \emph{memoryless} strategies,
where $\sigma(\omega)$ depends only on the last state of $\omega$,
in which case we define the strategy as a function 
$\sigma:S_\eitherplayer \rightarrow \dist(\act)$.
%The case of history-dependent strategies is an interesting topic for future research.
%(and \emph{history-dependent} if not). 
%% We use $MD^{\eitherplayer}_{\sgame}$ for
%% the set of memoryless deterministic strategies for player
%% $\eitherplayer\in\{\Box,\Diamond\}$ in $\sgame$; the sets $MR^{\eitherplayer}_{\sgame}$,
%% $HD^{\eitherplayer}_{\sgame}$, and $HR^{\eitherplayer}_{\sgame}$ are defined correspondingly.
%% Value of the game for property $P$, strategy $\sigma_1$ of the player $\Box$ and
%% strategy $\sigma_2$ of the player $\Diamond$ is a function $V^{\sigma_1,\sigma_2} : s \rightarrow \mathbb{R}$.
%% We denote valuations $V^{-,-}$ and $V^{+,+}$ when both players minimize/maximize.
We write $\strats_\sgame^\eitherplayer$ for the set of all (memoryless)
player $\eitherplayer$ strategies in $\sgame$.

%and $\strats_\sgame^{\eitherplayer,C}$ (where $C=\{\dete,\rand\}$)
%where we need to distinguish between those which are
%deterministic ($\dete$) and randomised ($\rand$).

%-------------------------------------------------------------------------

\subsection{Properties and Rewards}

In order to synthesise controllers, we need a formal description of their required properties.
In this paper, we use two common classes of properties:
\emph{probabilistic reachability} and \emph{expected total reward},
which we will express in an extended version of the temporal logic PCTL~\cite{HJ94}.
%and its extensions~\cite{FKNP11}.

For probabilistic reachability, we write properties of the form $\phi = \calP_{\bowtie p}[\,\future g\,]$,
where $\bowtie\,\,\in\{\leq,\geq\}$, $p\in[0,1]$ and $g\subseteq S$ is a set of target states,
meaning that the probability of reaching a state in $g$ satisfies the bound $\bowtie p$.
Formally, for a specific pair of strategies
$\ctrlstrat\in\strats_\sgame^\Diamond, \envstrat\in\strats_\sgame^\Box$ for $\sgame$,
the probability of reaching $g$ under $\ctrlstrat$ and $\envstrat$ is
\[
\Prb_{\sgame,\sinit}^{\ctrlstrat,\envstrat}(\future g) \rmdef
\Prb_{\sgame,\sinit}^{\ctrlstrat,\envstrat}
(\{s_0 a_0 s_1 a_1 \dots\in\ipaths_\sinit\,|\, s_i\in g \mbox{ for some } i\}).
\]
We say that $\phi$ is satisfied under $\ctrlstrat$ and $\envstrat$,
denoted $\sgame,\ctrlstrat,\envstrat \models \phi$, if
$\Prb_{\sgame,\sinit}^{\ctrlstrat,\envstrat}(\future g) \bowtie p$.

%$$\Prb_{\sgame,\sinit}^{\ctrlstrat,\envstrat}(\{s_0 a_0 s_1 a_1 \dots\in\ipaths_\sinit\,|\, s_i\in T \mbox{ for some } i\}) \bowtie p$$

We also augment stochastic games with 
\emph{reward structures}, which are functions of the form
$r:S\times\act\to\Qset_{\ge 0}$ mapping state-action pairs to non-negative rationals.
In practice, we often use these to represent ``costs'' (e.g. elapsed time or energy consumption),
despite the terminology ``rewards''.
The restriction to non-negative rewards allows us to avoid problems with non-uniqueness
of total rewards, which would require special treatment \cite{TV87}.

%
Rewards are accumulated along a path and,
%The \emph{total reward} for a reward structure $r$ along an infinite path $\omega=s_0 a_0 s_1 a_1 \dots$
%is $\smash{r(\omega) \rmdef \sum_{j=0}^{\infty} r(s_j,a_j)}$.
for strategies
$\ctrlstrat\in\strats_\sgame^\Diamond$ and $\envstrat\in\strats_\sgame^\Box$,
the \emph{expected total reward} is defined as:
\[
E_{\sgame,\sinit}^{\ctrlstrat,\envstrat}(r) \rmdef\int_{\omega=s_0 a_0 s_1 a_1 \dots\in\ipaths_\sinit} \ \sum_{j=0}^{\infty} r(s_j,a_j) \,d\Prb_{\sgame,\sinit}^{\ctrlstrat,\envstrat}.
\]
For technical reasons, we will always assume the maximum possible reward
$\sup_{\sigma,\pi}E_{\sgame,s}^{\ctrlstrat,\envstrat}(r)$ is finite
(which can be checked with an analysis of the game's underlying graph); similar assumptions are commonly introduced~\cite[Section 7]{Put94}.
In our proofs, we will also use $E_{\sgame,\sinit}^{\ctrlstrat,\envstrat}(r{\downarrow}s)$ for the expected total reward accumulated before the first visit to $s$, defined by:
\[
 E_{\sgame,\sinit}^{\ctrlstrat,\envstrat}(r{\downarrow}s) \rmdef\int_{\omega=s_0 a_0 s_1 a_1\ldots\in\ipaths_\sinit}\sum_{i=0}^{\mathit{fst}(s,\omega)-1} r(s_i,a_i)\,d\Prb_{\sgame,\sinit}^{\ctrlstrat,\envstrat}
\]
where $\mathit{fst}(s,\omega)$ is $\min\{i \mid s_i = s\}$ if $\omega=s_0 a_0 s_1 a_1\ldots$ contains $s_i$, and $\infty$ otherwise.

An expected reward property is written $\phi = \propbt{r}{b}$ (where $\mathtt{C}$ stands for \emph{cumulative}),
meaning that the expected total reward for $r$ satisfies $\bowtie b$.
%Using the same notation as for probabilistic reachability,
We say that $\phi$ is satisfied under strategies $\ctrlstrat$ and $\envstrat$,
denoted $\sgame,\ctrlstrat,\envstrat \models \phi$, if
$E_{\sgame,\sinit}^{\ctrlstrat,\envstrat}(r) \bowtie b$.

In fact, probabilistic reachability can easily be reduced to expected total reward
(by replacing any outgoing transitions from states in the target set
with a single transition to a sink state labelled with a reward of 1).
Thus, in the techniques presented in this paper,
we focus purely on expected total reward.

%-------------------------------------------------------------------------

\subsection{Controller Synthesis}

To perform controller synthesis, we model the system as a stochastic game $\sgame=\gametuple$,
where player $\Diamond$ represents the controller and player $\Box$ represents the environment.
A specification of the required behaviour of the system is a property $\phi$,
either a probabilistic reachability property $\calP_{\bowtie p}[\,\future g\,]$
or an expected total reward property $\propbt{r}{b}$.

%The classical \emph{controller synthesis} problem asks whether there exists
%a controller strategy $\ctrlstrat\in\strats_\sgame^\Diamond$
%such that $\sgame,\ctrlstrat,\envstrat \models \phi$ for any possible
%environment strategy $\envstrat\in\strats_\sgame^\Box$.
%We call such a strategy \emph{sound}.
%
\begin{defi}[Sound strategy]\label{defn:soundstrat}
A strategy $\ctrlstrat\in\strats_\sgame^\Diamond$
for player $\Diamond$ in stochastic game $\sgame$
is \emph{sound} for a property $\phi$ if $\sgame,\ctrlstrat,\envstrat \models \phi$
for any strategy $\envstrat\in\strats_\sgame^\Box$.
\end{defi}
%
To simplify notation, we will consistently use $\ctrlstrat$ and $\envstrat$ to refer to strategies
of player $\Diamond$ and $\Box$, respectively,
and will not always state explicitly that
$\ctrlstrat\in\strats_\sgame^\Diamond$ and $\envstrat\in\strats_\sgame^\Box$.
%
Notice that, in \defref{defn:soundstrat}, strategies $\ctrlstrat$ and $\envstrat$ are both memoryless.
We could equivalently allow $\envstrat$ to range over history-dependent strategies
since, for the properties $\phi$ considered in this paper
(probabilistic reachability and expected total reward),
the existence of a history-dependent counter-strategy $\envstrat$ for which $\sgame,\ctrlstrat,\envstrat \not\models \phi$
implies the existence of a memoryless one.

The classical \emph{controller synthesis} problem asks whether there exists a sound strategy
for game $\sgame$ and property $\phi$. We can determine whether this is the case
by computing the optimal strategy for player $\Diamond$ in $\sgame$~\cite{Con93,FV97}.
This problem is known to be in NP $\cap$ co-NP, but, in practice,
methods such as value or policy iteration can be used efficiently.

%-------------------------------------------------------------------------

\begin{figure}
  \centering
  %\vspace*{-0.8cm}
  \input{fig_running_game}
  %\vspace*{-0.5cm}
  \caption{A stochastic game $\sgame$ used as a running example (see \egref{eg:game}).}
  \label{fig:running_game}
  %\vspace*{-1.6em}
\end{figure}

%-------------------------------------------------------------------------

\begin{examp}\label{eg:game}
\figref{fig:running_game} shows a stochastic game $\sgame$, %, which we will use as a running example.
with controller and environment player states drawn as diamonds and squares, respectively.
It models the control of a robot moving between 4 locations ($s_0,s_2,s_3,s_5$).
When moving east ($s_0{\ra}s_2$ or $s_3{\ra}s_5$), it may be impeded by a second robot,
depending on the position of the latter.
If it is impeded, there is a chance that it does not successfully move to the next location.

We use a reward structure $\mathit{moves}$, which assigns 1 to the controller actions
$\mathit{north}$, $\mathit{east}$, $\mathit{south}$,
and define property $\phi=\nprop{\mathit{moves}}{5}$,
meaning that the expected number of moves to reach $s_5$ is at most 5
(notice that $s_5$ is the only state from which all subsequent transitions have reward zero).
A sound strategy for $\phi$ in $\sgame$ (found by minimising $\mathit{moves}$)
chooses $\mathit{south}$ in $s_0$ and $\mathit{east}$ in $s_3$,
yielding an expected number of moves of $3.5$.
\end{examp}
%\vspace*{-6pt}

%-------------------------------------------------------------------------

